A Game-Theoretic Approach for Security Control Selection

Selecting the combination of security controls that will most effectively protect a system's assets is a difficult task. If the wrong controls are selected, the system may be left vulnerable to cyber-attacks that can impact the confidentiality, integrity and availability of critical data and services. In practical settings, it is not possible to select and implement every control possible. Instead considerations, such as budget, effectiveness, and dependencies among various controls, must be considered to choose a combination of security controls that best achieve a set of system security objectives. In this paper, we propose a game-theoretic approach for selecting effective combinations of security controls based on expected attacker profiles and a set budget. The control selection problem is set up as a two-person zero-sum one-shot game. Valid control combinations for selection are generated using an algebraic formalism to account for dependencies among selected controls. We demonstrate the proposed approach on an illustrative financial system used in government departments under four different scenarios. The results illustrate how a security analyst can use the proposed approach to guide and support decision-making in the control selection activity when developing secure systems.

==> eptcsdata.tex <==
\providecommand{\firstpage}{103}
\providecommand{\publicationstatus}{A. Achilleos and A. Francalanza (Eds.): Fifteenth\\ International Symposium on Games, Automata, Logics,\\ and Formal Verification (GandALF 2024).\\
EPTCS 409, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.409.11}{10.4204/EPTCS.409.11}}
\pdfoutput=1

